A Study of Network Congestion in Two Supercomputing High-Speed Interconnects

Network congestion in high-speed interconnects is a major source of application run time performance variation. Recent years have witnessed a surge of interest from both academia and industry in the development of novel approaches for congestion control at the network level and in application placement, mapping, and scheduling at the system-level. However, these studies are based on proxy applications and benchmarks that are not representative of field-congestion characteristics of high-speed interconnects. To address this gap, we present (a) an end-to-end framework for monitoring and analysis to support long-term field-congestion characterization studies, and (b) an empirical study of network congestion in petascale systems across two different interconnect technologies: (i) Cray Gemini, which uses a 3-D torus topology, and (ii) Cray Aries, which uses the DragonFly topology.

==> background.tex <==
\section{Background and Motivation}
\label{s:motivation}

==> char.tex <==
\section{Characterization}
\label{s:char}




\subsection{Runtimes}
\includegraphics[width=0.5\textwidth]{runtimes.png}
Y axis shows wall time for HAMR (the victim application in experiments) runs. The X axis represents configuration in which the application ran (BS - block spread and IS - interleave spread).
\subsection{Symmetric Group Links}
\includegraphics[width=0.5\textwidth]{symmetric.png}
The Aries interconnect implements Universal Globally-Adaptive Load-Balanced (UGAL) routing which estimates congestion on global links and routes traffic to balance global congestion. A flit can be routed to it's destination switch using a minimal route (across a single global link) or a non-minimal route (across two global links). There are multiple possibilities for non-minimal routes and under ideal stable state conditions each of those routes are utilized equally. Errors in approximation of global congestion could lead to unequal utilization of these routes. In the experimental setup two applications were running occupying three cabinets. In such an application placement three cabinets in the first group and three cabinets in the second group are symmetrical to each other i.e. all corresponding blue, black and green links are identically connected with respect to the applications. In other words with respect to the view of apps the symmetric links are identical and lie on non-minimal routes. The unequal distribution of traffic on these links indicate issues in UGAL routing. The following graphs shows the distribution of differences between maximum and minimum $P_{TS}$ for each symmetrical group.
The X axis represents difference between minimum and maximum PTS values for each symmetrical group across all measurements.
The Y axis represents the inverse CDF value.
\subsection{Hotpsot Links}
\includegraphics[width=0.5\textwidth]{hotspot_aries.pdf}
The X axis represents cut off in terms of PTS(\%) for a link to be considered as congested. The Y axis shows percentile of duration for varying cut offs of PTS.
